3D Denoisers are Good 2D Teachers: Molecular Pretraining via Denoising and Cross-Modal Distillation

Pretraining molecular representations from large unlabeled data is essential for molecular property prediction due to the high cost of obtaining ground-truth labels. While there exist various 2D graph-based molecular pretraining approaches, these methods struggle to show statistically significant gains in predictive performance. Recent work have thus instead proposed 3D conformer-based pretraining under the task of denoising, which led to promising results. During downstream finetuning, however, models trained with 3D conformers require accurate atom-coordinates of previously unseen molecules, which are computationally expensive to acquire at scale. In light of this limitation, we propose D&D, a self-supervised molecular representation learning framework that pretrains a 2D graph encoder by distilling representations from a 3D denoiser. With denoising followed by cross-modal knowledge distillation, our approach enjoys use of knowledge obtained from denoising as well as painless application to downstream tasks with no access to accurate conformers. Experiments on real-world molecular property prediction datasets show that the graph encoder trained via D&D can infer 3D information based on the 2D graph and shows superior performance and label-efficiency against other baselines.

==> figures/ablation_label_averaged.tex <==
\begin{figure*}[!ht]
\centering
\begin{subfigure}[b]{0.495\textwidth}
    \centering
    \includegraphics[width=\textwidth]{example-image-a}
    \caption{{OGB}}    
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.495\textwidth}
    \centering
    \includegraphics[width=\textwidth]{example-image-a}
    \caption{{Custom}}    
\end{subfigure}
\caption{Label-efficiency experimental results. X-axis shows what percentage of the training data was used, and Y-axis shows performance on the test set.} 
\label{fig:mean and std of nets}
\end{figure*}

==> tables/ablation_arch_table.tex <==
\begin{table}[ht]
    \centering
    \caption{Performance in OGB and customized datasets with varying 2D-graph encoder architecture.\sungjun{Hopefully, our method shows significant improvement in an model-agnostic manner. Low priority: experiments might take a while to setup}} \label{tab:ablation_arch}
    \resizebox{.5\textwidth}{!}{\begin{tabular}{l|cccc}
        \toprule
        Dataset & GIN~\cite{xu2018gin} & Graphormer~\cite{ying2021graphormer} & TokenGT~\cite{kim2022tokengt}\\
        \midrule
        No pretrain &  &  & \\
        PDF (ours) &  &  &  \\
        \bottomrule
    \end{tabular}
    } 
\end{table}

==> tables/ablation_distillation_table.tex <==
\begin{table}[ht]
    \centering
    \caption{Performance in OGB and customized datasets with and without 3D-pretraining via denoising.} \label{tab:ablation_denoising} 
    \vspace{.1in}
    \resizebox{.5\textwidth}{!}{\begin{tabular}{c|cc}
        \toprule
        Method & OGB & Custom\\
        \midrule
        No Pretraining + Node-distillation &  & \\
        Contrastive + Node-distillation &  & \\
        Denoising + Graph-distillation &  & \\
        \midrule
        Denoising + Node-distillation (ours) &  & \\
        \bottomrule
    \end{tabular}
    }
\end{table}

==> tables/ablation_label_table.tex <==
\begin{table}[ht]
    \centering
    \caption{Performance in OGB with increasing size of finetuning training sets. \sungjun{probably better off having this as a line plot (x-axis: percentage / y-axis: performance), but the scales for different issue $\to$ maybe average only the roc-auc benchmarks and compare between 1) no pretrain 2) 3d infomax 3) our method.}} \label{tab:ablation_label} 
    \resizebox{.5\textwidth}{!}{\begin{tabular}{lr|ccccc}
        \toprule
        Dataset & Metric & 20\% & 40\% & 60\% & 80\% & 100\% \\
        \midrule
        ESOL & RMSE($\downarrow$) &  &  &  &  &  \\
        FREESOLV & RMSE($\downarrow$) &  &  &  &  &  \\
        LIPO & RMSE($\downarrow$) &  &  &  &  &  \\
        MUV & AP($\uparrow$) &  &  &  &  &  \\
        PCBA & AP($\uparrow$) &  &  &  &  &  \\
        BACE & ROC-AUC($\uparrow$) &  &  &  &  &  \\
        BBBP & ROC-AUC($\uparrow$) &  &  &  &  &  \\
        CLINTOX & ROC-AUC($\uparrow$) &  &  &  &  &  \\
        HIV & ROC-AUC($\uparrow$) &  &  &  &  &  \\
        SIDER & ROC-AUC($\uparrow$) &  &  &  &  &  \\
        TOX21 & ROC-AUC($\uparrow$) &  &  &  &  &  \\
        TOXCAST & ROC-AUC($\uparrow$) &  &  &  &  &  \\
        \bottomrule
    \end{tabular}
    }
\end{table}

==> tables/custom_table.tex <==
\begin{table}[ht]
    \centering
    \caption{Custom Dataset Results. Performance is measured in L1 loss (lower is better).} \label{tab:custom_l1} 
    \vspace{.1in}
    \resizebox{.5\textwidth}{!}{\begin{tabular}{l|cccc}
        \toprule
        Dataset & NP (mean) & NP (VN) & PDF (mean) & PDF (VN)\\
        \midrule
        BP & 0.3314 & 0.3353 & 0.2922 & \bf 0.2293\\
        MP & 0.3703 & 0.3713 & 0.3703 & \bf 0.2994\\
        RI & 0.1476 & 0.1489 & 0.1221 & \bf 0.0678\\
        logP & 0.0486 & 0.0521 & 0.0486 & \bf 0.0230\\
        \bottomrule
    \end{tabular}
    }
\end{table}


\begin{table}[ht]
    \centering
    \caption{Custom Dataset Results. Performance is measured in $R^2$ correlation score (higher is better).} \label{tab:custom_r2} 
    \vspace{.1in}
    \resizebox{.5\textwidth}{!}{\begin{tabular}{l|cccc}
        \toprule
        Dataset & NP (mean) & NP (VN) & PDF (mean) & PDF (VN)\\
        \midrule
        BP & 0.6206 & 0.6371 & 0.6698 & \bf 0.6889\\
        MP & 0.6929 & 0.6891 & 0.6929 & \bf 0.8115\\
        RI & 0.9325 & 0.9366 & 0.9493 & \bf 0.9815\\
        logP & 0.9938 & 0.9938 & 0.9938 & \bf 0.9977\\
        \bottomrule
    \end{tabular}
    }
\end{table}

==> tables/ogb_table.tex <==
\begin{table}[ht]
    \centering
    \caption{OGB Results. Finetuning the model after SSL via \ourmethod{} leads to consistently higher performance in 11 out of 12 datasets in the OGB benchmark.} \label{tab:ogb} 
    \vspace{.1in}
    \resizebox{.5\textwidth}{!}{\begin{tabular}{lr|cc|cc}
        \toprule
        Dataset & Metric & NP (mean) & NP (VN) & PDF (mean) & PDF (VN)\\
        \midrule
        ESOL & RMSE($\downarrow$) & 1.1629 & 1.1334 & 1.0712 & \bf 1.0224\\
        FREESOLV & RMSE($\downarrow$) & 3.8126 & 3.7088 & 3.5261 & \bf 3.5233\\
        LIPO & RMSE($\downarrow$) & 0.9663 & 0.9669 & \bf 0.6777 & 0.7219\\
        MUV & AP($\uparrow$) & 0.02955 & 0.02906 & 0.04591 & \bf 0.07247\\
        PCBA & AP($\uparrow$) & 0.1565 & 0.1493 & 0.2515 & \bf 0.2626\\
        BACE & ROC-AUC($\uparrow$) & 0.7606 & \bf 0.7943 & 0.7470 & 0.7893\\
        BBBP & ROC-AUC($\uparrow$) & 0.6410 & 0.6263 & \bf 0.7049 & 0.6645\\
        CLINTOX & ROC-AUC($\uparrow$) & 0.6024 & 0.6009 & 0.6538 & \bf 0.6915\\
        HIV & ROC-AUC($\uparrow$) & 0.7032 & 0.6956 & \bf 0.7675 & 0.7663\\
        SIDER & ROC-AUC($\uparrow$) & 0.5994 & 0.6000 & 0.6265 & \bf 0.6307\\
        TOX21 & ROC-AUC($\uparrow$) & 0.7259 & 0.7281 & \bf 0.7605 & 0.7527\\
        TOXCAST & ROC-AUC($\uparrow$) & 0.6270 & 0.6188 & 0.6562 & \bf 0.6580\\
        \bottomrule
    \end{tabular}
    }
\end{table}

==> tables/vs_3dinfomax_ogb.tex <==
\begin{table}[!ht]
    \centering
    \caption{Test evaluation results on each OGB non-quantum property prediction dataset.}\label{tab:vs_3dinfomax_ogb} 
    \vspace{.1in}
    \resizebox{\textwidth}{!}{\begin{tabular}{l|cccccccccc}
        \toprule
        Target & ESOL & FREESOLV & LIPO & BACE & BBBP & CLINTOX & HIV & SIDER & TOX21 & TOXCAST \\
        Metric & RMSE($\downarrow$) & RMSE($\downarrow$) & RMSE($\downarrow$) & ROC-AUC($\uparrow$) & ROC-AUC($\uparrow$) & ROC-AUC($\uparrow$) & ROC-AUC($\uparrow$) & ROC-AUC($\uparrow$) & ROC-AUC($\uparrow$) & ROC-AUC($\uparrow$)\\
        \midrule
        \textsc{RandInit} & 0.947{\scriptsize $\pm$0.038} & \bf 2.233{\scriptsize $\pm$0.261} & 0.739{\scriptsize $\pm$0.001} & 78.13{\scriptsize $\pm$1.30} & 68.27{\scriptsize $\pm$1.98} & 58.98{\scriptsize $\pm$5.40} & \bf 77.06{\scriptsize $\pm$3.16} & 55.95{\scriptsize $\pm$3.27} & 73.88{\scriptsize $\pm$0.64} & 63.62{\scriptsize $\pm$0.48} \\
        \textsc{GraphCL} & 0.959{\scriptsize $\pm$0.047} & 3.744{\scriptsize $\pm$0.292} & 0.714{\scriptsize $\pm$0.011} & 77.18{\scriptsize $\pm$4.01} & \bf 71.06{\scriptsize $\pm$2.00} & 51.07{\scriptsize $\pm$5.52} & 76.06{\scriptsize $\pm$1.06} & 57.32{\scriptsize $\pm$5.00} & \bf 78.92{\scriptsize $\pm$0.61} & 64.95{\scriptsize $\pm$0.31} \\
        \textsc{DisPred} & 0.986{\scriptsize $\pm$0.025} & 2.486{\scriptsize $\pm$0.222} & 0.718{\scriptsize $\pm$0.021} & 76.51{\scriptsize $\pm$1.95} & 66.06{\scriptsize $\pm$1.84} & 55.77{\scriptsize $\pm$5.86} & 75.66{\scriptsize $\pm$1.26} & 57.13{\scriptsize $\pm$1.89} & 73.87{\scriptsize $\pm$0.43} & 61.58{\scriptsize $\pm$0.58} \\
        \textsc{ConfGen} & \bf 0.867{\scriptsize $\pm$0.045} & 2.428{\scriptsize $\pm$0.155} & 0.757{\scriptsize $\pm$0.035} & 80.02{\scriptsize $\pm$1.58} & 66.16{\scriptsize $\pm$2.24} & 64.27{\scriptsize $\pm$5.22} & 76.57{\scriptsize $\pm$1.39} & 56.34{\scriptsize $\pm$4.20} & 75.24{\scriptsize $\pm$1.00} & 64.74{\scriptsize $\pm$1.20} \\
        \textsc{3DInfomax} & 0.894{\scriptsize $\pm$0.028} & 2.337{\scriptsize $\pm$0.227} & \bf 0.695{\scriptsize $\pm$0.012} & 79.42{\scriptsize $\pm$1.94} & 69.10{\scriptsize $\pm$1.07} & 59.43{\scriptsize $\pm$3.21} & 76.08{\scriptsize $\pm$1.33} & 53.37{\scriptsize $\pm$3.34} & 74.46{\scriptsize $\pm$0.74} & 64.41{\scriptsize $\pm$0.88} \\
        \midrule
        %\textsc{RandInit} & \bf 0.8802{\scriptsize $\pm$0.0966} & 2.5854{\scriptsize $\pm$0.5983} & 1.4936{\scriptsize $\pm$1.3587} & \bf 81.92{\scriptsize $\pm$2.95} & 66.47{\scriptsize $\pm$1.59} & 86.64{\scriptsize $\pm$2.64} & 77.13{\scriptsize $\pm$1.21} & 60.88{\scriptsize $\pm$3.00} & 75.07{\scriptsize $\pm$0.63} & 66.33{\scriptsize $\pm$0.78} \\
        %\textsc{3DInfomax} & 0.9474{\scriptsize $\pm$0.0309} & 4.4483{\scriptsize $\pm$1.5230} & 0.7000{\scriptsize $\pm$0.0124} & 74.87{\scriptsize $\pm$5.76} & \bf 70.66{\scriptsize $\pm$1.77} & 86.32{\scriptsize $\pm$4.18} & 76.36{\scriptsize $\pm$3.29} & \bf 61.20{\scriptsize $\pm$1.25} & 75.85{\scriptsize $\pm$0.64} & \bf 67.29{\scriptsize $\pm$1.05} \\
        %\textsc{DnD-Graph} & 1.0041{\scriptsize $\pm$0.0904} & 2.4907{\scriptsize $\pm$0.3689} & 0.7089{\scriptsize $\pm$0.0372} & 78.38{\scriptsize $\pm$4.39} & 67.49{\scriptsize $\pm$3.29} & 87.68{\scriptsize $\pm$4.06} & \bf 77.30{\scriptsize $\pm$1.20} & 58.52{\scriptsize $\pm$1.72} & 75.90{\scriptsize $\pm$0.66} & 66.85{\scriptsize $\pm$0.39} \\
        %\textsc{DnD-Node} & 0.9357{\scriptsize $\pm$0.0247} & \bf 2.4765{\scriptsize $\pm$0.2325} & \bf 0.6816{\scriptsize $\pm$0.0114} & 80.74{\scriptsize $\pm$2.49} & 67.03{\scriptsize $\pm$2.25} & \bf 88.11{\scriptsize $\pm$3.44} & 74.53{\scriptsize $\pm$1.37} & 57.34{\scriptsize $\pm$1.89} & \bf 75.99{\scriptsize $\pm$0.69} & 66.68{\scriptsize $\pm$0.29} \\
        \textsc{DnD-Graph} & 0.873{\scriptsize $\pm$0.030} & 2.362{\scriptsize $\pm$0.277} & 0.721{\scriptsize $\pm$0.067} & 79.28{\scriptsize $\pm$2.49} & 67.47{\scriptsize $\pm$2.24} & \bf 89.10{\scriptsize $\pm$1.58} & 76.35{\scriptsize $\pm$0.99} & \bf 59.85{\scriptsize $\pm$1.95}  & 74.92{\scriptsize $\pm$1.05} & \bf 66.14{\scriptsize $\pm$0.63}\\
        \textsc{DnD-Node} & 0.879{\scriptsize $\pm$0.046} & 2.405{\scriptsize $\pm$0.327} & 0.700{\scriptsize $\pm$0.013} & \bf 80.60{\scriptsize $\pm$2.72} & 67.64{\scriptsize $\pm$2.36} & 87.22{\scriptsize $\pm$3.94} & 76.28{\scriptsize $\pm$1.61} & 59.40{\scriptsize $\pm$3.29} & 75.87{\scriptsize $\pm$0.95} & 65.49{\scriptsize $\pm$0.82}\\
        \bottomrule
    \end{tabular}
    }
\end{table}


